Analysis of Regression Discontinuity Designs with Multiple Cutoffs or Multiple Scores

We introduce the \texttt{Stata} (and \texttt{R}) package \texttt{rdmulti}, which includes three commands (\texttt{rdmc}, \texttt{rdmcplot}, \texttt{rdms}) for analyzing Regression Discontinuity (RD) designs with multiple cutoffs or multiple scores. The command \texttt{rdmc} applies to non-cumulative and cumulative multi-cutoff RD settings. It calculates pooled and cutoff-specific RD treatment effects, and provides robust bias-corrected inference procedures. Post estimation and inference is allowed. The command \texttt{rdmcplot} offers RD plots for multi-cutoff settings. Finally, the command \texttt{rdms} concerns multi-score settings, covering in particular cumulative cutoffs and two running variables contexts. It also calculates pooled and cutoff-specific RD treatment effects, provides robust bias-corrected inference procedures, and allows for post-estimation estimation and inference. These commands employ the \texttt{Stata} (and \texttt{R}) package \texttt{rdrobust} for plotting, estimation, and inference. Companion \texttt{R} functions with the same syntax and capabilities are provided.

==> code/output/rdmc_out5.log.tex <==
. rdmc y x, c(c) plot
{\smallskip}
{\smallskip}
Cutoff-specific RD estimation with robust bias-corrected inference
\HLI{12}{\TOPT}\HLI{67}
      Cutoff{\VBAR}    Coef.    P>|z|  [95\% Conf. Int.]     hl     hr      Nh   Weight
\HLI{12}{\PLUS}\HLI{67}
          33{\VBAR}  484.831    0.00    421.18  552.53    14.66  14.66    289    0.540
          66{\VBAR}  297.981    0.00    220.35  362.27    11.95  11.95    246    0.460
\HLI{12}{\PLUS}\HLI{67}
    Weighted{\VBAR}  398.915    0.00    348.74  445.14        .      .    535        .
      Pooled{\VBAR}  436.400    0.00    179.34  676.63    13.68  13.68    550        .
\HLI{12}{\BOTT}\HLI{67}


==> code/output/rdmc_out8.log.tex <==
. rdmcplot y x, c(c) nobins

